SoFFT: Spatial Fourier Transform for Modeling Continuum Soft Robots

Continuum soft robots, composed of flexible materials, exhibit theoretically infinite degrees of freedom, enabling notable adaptability in unstructured environments. Cosserat Rod Theory has emerged as a prominent framework for modeling these robots efficiently, representing continuum soft robots as time-varying curves, known as backbones. In this work, we propose viewing the robot's backbone as a signal in space and time, applying the Fourier transform to describe its deformation compactly. This approach unifies existing modeling strategies within the Cosserat Rod Theory framework, offering insights into commonly used heuristic methods. Moreover, the Fourier transform enables the development of a data-driven methodology to experimentally capture the robot's deformation. The proposed approach is validated through numerical simulations and experiments on a real-world prototype, demonstrating a reduction in the degrees of freedom while preserving the accuracy of the deformation representation.

==> biographies/daniele.tex <==
earned his M.Sc. degree in Robotics and Automation Engineering from the University of Pisa, Italy, in 2022. He is currently pursuing a Ph.D. in Biorobotics at Scuola Superiore Sant'Anna, Pisa, Italy, since 2022. 

His research focuses on model-based control of continuum soft robots.

==> biographies/diego.tex <==
earned his M.Sc. degree in Mechanical Engineering from the University of L'Aquila in 2021. Since 2022, he has been pursuing his Ph.D. at the BioRobotics Institute of Scuola Superiore Sant'Anna in Pisa, Italy. His research focuses on the development of learning-based control algorithms and the design of soft robotic systems.

==> biographies/egidio_falotico.tex <==
received the Graduate degree in computer sciences from the University of Pisa, Pisa, Italy, in 2008 and the Ph.D. degree in biorobotics with the Scuola Superiore Sant'Anna (SSSA), Pisa, Italy, in 2013, and the Ph.D. degree in cognitive sciences from the University Pierre et Marie Curie, Paris, France, in 2013.
He is currently an Assistant Professor with The BioRobotics Institute, SSSA, Pontedera, Italy. He is the author or coauthor of more than 100 international peer-reviewed papers and he regularly serves as a reviewer for more than ten international ISI journals. He served as PI for SSSA in EU-funded projects (Human Brain Project, Proboscis, Growbot), focusing on the development of brain-inspired algorithms for robot control and on machine learning models for soft robot control. His research interests focus on neurorobotics, i.e., the implementation of brain models from neuroscience in robots.

==> biographies/franco_angelini.tex <==
received the B.S. degree in com-
puter engineering in 2013 and M.S. degree (cum
laude) in automation and robotics engineering in
2016 from the University of Pisa, Pisa, Italy. The
University of Pisa also granted him a Ph.D. degree
(cum laude) in robotics in 2020 for which he was
awarded the 2021 SIDRA Award for the best PhD
Thesis in the area of Systems and Control Engineer-
ing at an Italian University. Franco is currently an
Assistant Professor at the University of Pisa. His
main research interests are control of soft robotic
systems, impedance planning, and robotic environmental monitoring.

==> sections/biography.tex <==
% biography section
% 
% If you have an EPS/PDF photo (graphicx package needed) extra braces are
% needed around the contents of the optional argument to biography to prevent
% the LaTeX parser from getting confused when it sees the complicated
% \includegraphics command within an optional argument. (You could create
% your own custom macro containing the \includegraphics command to make things
% simpler here.)
%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mshell}}]{Michael Shell}
% or if you just want to reserve a space for a photo:

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors_pics/daniele_caradonna.jpg}}]{Daniele Caradonna}
\input{biographies/daniele}
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors_pics/diego_bianchi.jpg}}]{Diego Bianchi}
\input{biographies/diego}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors_pics/franco.jpg}}]{Franco Angelini}
\input{biographies/franco_angelini}
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{imgs/authors_pics/egidio_falotico.png}}]{Egidio Falotico}
\input{biographies/egidio_falotico}
\end{IEEEbiography}

% if you will not have a photo at all:
% \begin{IEEEbiographynophoto}{John Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% insert where needed to balance the two columns on the last page with
% biographies
%\newpage

% \begin{IEEEbiographynophoto}{Jane Doe}
% Biography text here.
% \end{IEEEbiographynophoto}

% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}

==> sections/regressor_identification.tex <==
%%% Identification %%%
\subsection{Parametric Identification \textcolor{red}{Doesn't Work :(}}
To identify the physical parameters of the robot, we can expand the regressor-driven method proposed in \cite{stella2022experimental}, in the case of \ac{GVS} model. From the experimental data $\bm{\xi}(n \lambda_s, m T_s)$ and fixed a functional basis, we can fit the data, obtaining the experimental configurations $\bm{q}_{\textnormal{exp}}$. Assuming known the density $\rho$, and $E$, $\beta$ constant along the rod's length, we can reorganize the dynamics such as
\begin{equation} \label{eq:regressor}
    \bm{\delta}_m\left(\bm{q}, \dot{\bm{q}}, \ddot{\bm{q}}, \bm{\tau}\right) = \bm{Y}_m\left(\bm{q}, \dot{\bm{q}}\right) \bm{\pi} \quad \forall \, m \in [0, \, M - 1] \, ,
\end{equation}
where $\bm{Y}_m\left(\bm{q}, \dot{\bm{q}}\right) = - \begin{bmatrix}\bar{\bm{K}}\bm{q} & \bar{\bm{D}}\dot{\bm{q}}\end{bmatrix}$, $\bar{\bm{K}} , \, \bar{\bm{D}}$ are the stiffness and damping matrix with unitary $E$ and $\beta$, $\bm{\delta}_m\left(\bm{q}, \dot{\bm{q}}, \ddot{\bm{q}}, \bm{\tau}\right) = \bm{M}\left(\bm{q}\right) \ddot{\bm{q}} + \bm{C}\left(\bm{q}, \dot{\bm{q}}\right) \dot{\bm{q}} + \bm{G}\left(\bm{q}\right) - \bm{B}\left(\bm{q}\right) \bm{\tau}$, the subscript $\left(\cdot\right)_{m}$ indicates the time sample $m T_s$, and $\bm{\pi} = \begin{bmatrix}
    E & \beta
\end{bmatrix}^{\top}$.

The best set of parameters can be found by solving a \ac{WLS} problem, such as
\begin{equation} \label{eq:wls_functional}
    \hat{\bm{\pi}} = \underset{\bm{\pi}}{\arg \, \min} \left\{\frac{1}{2}\left(\bm{\delta} - \bm{Y}\bm{\pi}\right)^{\top} \bm{W} \left(\bm{\delta} - \bm{Y}\bm{\pi}\right)\right\} \, ,
\end{equation}
where $\bm{Y} = \begin{bmatrix} \bm{Y}^{\top}_0 & \bm{Y}^{\top}_{1} & \dots & \bm{Y}^{\top}_{M - 1} \end{bmatrix}^{\top}$, $\bm{\delta} = \begin{bmatrix} \bm{\delta}^{\top}_0 & \bm{\delta}^{\top}_{1} & \dots & \bm{\delta}^{\top}_{M - 1} \end{bmatrix}^{\top}$, and $\bm{W} \in \mathbb{R}^{\left(n \cdot M\right) \times \left(n \cdot M\right)}$. The weight matrix $\bm{W}$ allows us to give more importance to different strain modes or different time samples.

The solution of \eqref{eq:wls_functional} can be expressed as
\begin{equation} \label{eq:wsl_identification}
    \hat{\bm{\pi}} = \bm{Y}^{\dagger}_{\bm{W}} \, \bm{\delta} \, ,
\end{equation}
where $\bm{Y}^{\dagger}_{\bm{W}} = \left(\bm{Y}^{\top} \bm{W} \bm{Y}\right)^{-1} \bm{Y}^{\top} \bm{W}$ is the weighted Moore-Penrose left pseudoinverse.

==> tables/exp_table.tex <==
\begin{table}
\centering
\caption{Geometrical and estimated physical parameters of the H-Support Prototype}
\label{tab:exp_parameters}
    \begin{tabular}{lll}
    \toprule
    Name                    &   Symbol          &   Value                                                               \\
    \midrule
    Length                  &   $L$               &   \SI{0.192}{\meter}                                                            \\
    Cross-Section Radius               &   $R_{\textnormal{cs}}$               &   \SI{0.03}{\meter}                                                            \\
    Density                 &   $\bar{\rho}$    &   \SI{168.9179}{\kilogram/\meter^3}                                     \\     
    Young's Modulus         &   $E$             &   \SI{1.0}{M\pascal}                                             \\
    Poisson Ratio           &   $\nu$           &   0.5                                                                     \\
    Damping Coefficient                &   $\beta$         &   \SI{0.01}{M\pascal \cdot \second}         \\    
    \bottomrule
    \end{tabular}
\end{table}
